A Fair and Memory/Time-efficient Hashmap

Hashmap is a fundamental data structure in computer science. There has been extensive research on constructing hashmaps that minimize the number of collisions leading to efficient lookup query time. Recently, the data-dependant approaches, construct hashmaps tailored for a target data distribution that guarantee to uniformly distribute data across different buckets and hence minimize the collisions. Still, to the best of our knowledge, none of the existing technique guarantees group fairness among different groups of items stored in the hashmap. Therefore, in this paper, we introduce FairHash, a data-dependant hashmap that guarantees uniform distribution at the group-level across hash buckets, and hence, satisfies the statistical parity notion of group fairness. We formally define, three notions of fairness and, unlike existing work, FairHash satisfies all three of them simultaneously. We propose three families of algorithms to design fair hashmaps, suitable for different settings. Our ranking-based algorithms reduce the unfairness of data-dependant hashmaps without any memory-overhead. The cut-based algorithms guarantee zero-unfairness in all cases, irrespective of how the data is distributed, but those introduce an extra memory-overhead. Last but not least, the discrepancy-based algorithms enable trading off between various fairness notions. In addition to the theoretical analysis, we perform extensive experiments to evaluate the efficiency and efficacy of our algorithms on real datasets. Our results verify the superiority of FairHash compared to the other baselines on fairness at almost no performance cost.

==> _abstract.tex <==
\begin{abstract}
Hashing is a fundamental tool in computer science that is used to construct efficient indexes. There is a large amount of work constructing hashmaps trying to minimize the number of collisions leading to efficient lookup query time.
However, traditional hashmaps suffer from the fact that placing items to buckets uniformly at random does not often lead to a uniform/diverse realization where each bucket has roughly the same number of items.
As shown in~\cite{kraska2018case}, better data-dependent hashmaps can be learned with less conflicts.
Still, to the best of our knowledge the no data-dependent hashing technique guarantees group fairness among different groups of items stored in the hashmap. We are given a set $P$ of $n$ items and a family of groups $\Gee=\{\gee_1,\ldots, \gee_k\}$ such that every tuple $p\in P$ belongs to a unique group in $\Gee$.
Our first contribution is to formally define the fair hashing problem: Construct a hashmap with $m$ buckets such that, for every group $\gee_i\in \Gee$, every bucket contains (roughly) the same number of items from $\gee_i$. 

We propose two families of algorithms to design fair hashmaps. In the first family, we focus on hashmaps with optimum memory consumption (store only $m-1$ boundary points) minimizing the unfairness. We model the input tuples as points in $\Re^d$ and the goal is to find the vector $w\in \Re^d$ such that the projection of $P$ onto $w$ creates a ``convenient'' ordering to create a fair hashmap.
%For each projection, that consists of tuples in $\Re^1$, we design efficient algorithms that find near optimum partitions of exactly (or at most) $m$ buckets. Since the ranking-based algorithms need to visit $O(n^d)$ different vectors to find the best one, they are expensive, so we also propose a faster (linear on $n$) sampling-based algorithm that returns a hashmap with near-optimum fairness and optimum storage with high probability.
In the second family, we focus on hashmaps with $0$-unfairness, minimizing the memory consumption. We make the important observation, that the fair hashmap problem is reduced to the \emph{necklace splitting problem} and
%By carefully implementing algorithms for solving the necklace splitting problem,
we propose fast algorithms constructing hashmaps with $0$-unfairness using bounded memory. Finally, we implement our new algorithms and test their efficiency and efficacy on real datasets. We show that our hashmap implementation significantly reduces the unfairness compared to other baselines.
\end{abstract}

==> algs/nl2d.tex <==
\begin{algorithm}[!tb]
    \caption{\necklaceb} \label{alg:nl2d}
    \begin{algorithmic}[1] \small
    \Require{The set of points $P$ (with two groups $\{\gee_1,\gee_2\}$)}
    \Ensure{Bin boundaries $B$ and corresponding buckets $H$}
        \State $C=\langle p_1,p_2,\cdots,p_n\rangle\gets$ {\bf sort} $P$ based on an attribute $x$
        % \State $C\gets$ {\bf circle}$(\langle p_1,p_2,\cdots,p_n\rangle)$ {\tt\small //make the list circular}
        \State cuts $\gets$ {\bf new set}$()$; ~$j\gets 0$; $bkt\gets 0$; init $\gets$ {\bf true}
        \While{$|C|>0$} 
        \Statex{\tt\small //current window is in range $\Big[C[j],C\big[(j+\frac{n}{m})\% |C|\big]\Big]$}
            \If{init == {\bf true}} {\tt\small count \#$\gee_1$ in the window}
                \State $\sigma_1\gets 0$; ~init $\gets$ {\bf false}
                \For{$i=1$ to $\frac{n}{m}$}
                    \State {\bf if} $\gee(C\big[(i+j)\% |C|\big])==\gee_1$ {\bf then} $\sigma_1++$
                \EndFor
            \EndIf
            \If{$\sigma_1==\frac{|\gee_1|}{m}$} {\tt\small // new cut found}
                \State cuts $\gets$ cuts $\cup \big\{(j-1)\% |C|, (j+\frac{n}{m})\% |C|\big\}$
                \State {\tt\small //remove all points in the window from $C$}
                \For{($i=0$ to $\frac{n}{m}$ with step $(i++)\%|C|$)}
                    \State $H^{tmp}_{C[j]}\gets bkt$; {\bf remove}$(C[j])$
                \EndFor
                \State $bkt\gets bkt+1$; init $\gets$ {\bf true}
            \EndIf            
        \EndWhile
        \State {\bf sort}$($cuts$)$
        \For{$j=0$ to |cuts|}
            \State let $p_i = C[j]$
            \State $B_j=\frac{p_i[x]+p_{i+1}[x]}{2}$;  {\tt\small // the right boundary of the $j$-th bin}
            \State $H_j\gets H^{tmp}_i$; {\tt\small // the bucket assigned to the $j$-th bin}
        \EndFor
        \State {\bf return} $(B,H)$
    \end{algorithmic}
\end{algorithm}

==> bhaskar-header.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% if using simple latex comment the following two lines 
%%\usepackage{fontspec} % use xelatex to pdf
%%\setmainfont{Times New Roman} % use xelatex to pdf
\usepackage{times}
\usepackage{mathpazo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{changepage}   % for the adjustwidth environment
\usepackage{sidecap}
\usepackage{frcursive}
%%\usepackage[T1]{fontenc}
\usepackage{setspace}
\usepackage{caption}
% code to define \subsubsubsection etc.
\usepackage{titlesec}
\usepackage[multiple]{footmisc}
\usepackage{multirow}

%\usepackage[mathscr]{eucal}

\titleclass{\subsubsubsection}{straight}[\subsection]

\newcounter{subsubsubsection}[subsubsection]
\renewcommand\thesubsubsubsection{\thesubsubsection.\arabic{subsubsubsection}}
\renewcommand\theparagraph{\thesubsubsubsection.\arabic{paragraph}} % optional; useful if paragraphs are to be numbered

\titleformat{\subsubsubsection}
  {\normalfont\normalsize\bfseries}{\thesubsubsubsection}{1em}{}
\titlespacing*{\subsubsubsection}
{0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}

\makeatletter
\renewcommand\paragraph{\@startsection{paragraph}{5}{\z@}%
  {3.25ex \@plus1ex \@minus.2ex}%
  {-1em}%
  {\normalfont\normalsize\bfseries}}
\renewcommand\subparagraph{\@startsection{subparagraph}{6}{\parindent}%
  {3.25ex \@plus1ex \@minus .2ex}%
  {-1em}%
  {\normalfont\normalsize\bfseries}}
\def\toclevel@subsubsubsection{4}
\def\toclevel@paragraph{5}
\def\toclevel@paragraph{6}
\def\l@subsubsubsection{\@dottedtocline{4}{9em}{4em}}
\def\l@paragraph{\@dottedtocline{5}{10em}{5em}}
\def\l@subparagraph{\@dottedtocline{6}{14em}{6em}}
\makeatother

\setcounter{secnumdepth}{4}
\setcounter{tocdepth}{4}

%\usepackage{tikz}

%\usetikzlibrary{arrows}
%\usetikzlibrary{shapes}

%\newcommand{\mymk}[1]{%
  %\tikz[baseline=(char.base)]\node[anchor=south west, draw,rectangle, rounded corners, inner sep=2pt, minimum size=7mm,
    %text height=2mm](char){\ensuremath{#1}} ;}

%\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            %\node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

\usepackage{kbordermatrix,blkarray}

\renewcommand{\kbldelim}{(}
\renewcommand{\kbrdelim}{)}

\newcounter{subcount}

\usepackage{wrapfig}
\usepackage{colortbl}
\usepackage{etex}
\usepackage{bbding}
\usepackage{dingbat}
\usepackage[ruled]{algorithm2e}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{algorithmic}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{latexsym}
\usepackage{graphicx}
\usepackage{graphics}
\usepackage{color}
\usepackage[normalem]{ulem}
\usepackage{balance}
\usepackage{textcomp}
\usepackage{nicefrac}
\usepackage{wasysym}
\usepackage[inline]{enumitem}
\usepackage{gensymb}
\usepackage{ctable}
\usepackage{url}
\usepackage{longtable}
%%\usepackage{citesort}
\usepackage[numbers,sort&compress]{natbib}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% for removing extra default space for a figure in LaTex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% See p.105 of "TeX Unbound" for suggested values.
% See pp. 199-200 of Lamport's "LaTeX" book for details.
%   General parameters, for ALL pages:
\renewcommand\topfraction{.99}        % max fraction of floats at top
\renewcommand\bottomfraction{.99}     % max fraction of floats at bottom
\renewcommand\textfraction{.01}   
%   Parameters for TEXT pages (not float pages):
\setcounter{totalnumber}{2}
\setcounter{topnumber}{1}
\setcounter{bottomnumber}{1}
%   Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.99}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{pstricks,pst-node,pst-plot,pst-coil,pst-text,multido,pst-3d,pst-tree,pst-grad,graphics,graphicx}

\usepackage{pifont,epsfig,rotating}

\usepackage{etoolbox}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\usepackage{etaremune}

\usepackage{mathtools}

\setlength{\topmargin}{0in} 
\setlength{\oddsidemargin}{0.0in}
\setlength{\evensidemargin}{0.0in}
\setlength{\headheight}{0in} 
\setlength{\headsep}{0in} 
\setlength{\textheight}{9in}
\setlength{\textwidth}{6.5in}
\renewcommand{\baselinestretch}{1}

\definecolor{dgreyblue}{rgb}{0.26,0.3,0.46}             %89.25 102 158.10
\newcommand{\grey}[1]{{\textcolor{dgreyblue}{#1}}}
\newcommand{\truered}[1]{{\textcolor{red}{#1}}}
\newcommand{\bee}{{\mathbf{e}}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\R}{{\mathbb R}}  %ams bold
\newcommand{\PP}{{\mathbb P}}  %ams bold
\newcommand{\ip}[2]{\langle #1 , #2 \rangle}
\renewcommand{\text}[1]{\hbox{\rm \ #1\ \/}}
\newcommand{\card}[1]{\left|#1\right|}
\newcommand{\spa}{\mbox{span}\,}
\newcommand{\col}{\mbox{col}\,}
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beqn}{\begin{eqnarray*}}
\newcommand{\eeqn}{\end{eqnarray*}}
\newcommand{\beq}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\eps}{\varepsilon}
\newcommand{\abs}[1]{\left\vert #1 \right\vert}
\newcommand{\st}{\; | \;}
\newcommand{\eqmul}[2]{\begin{equation}\label{#1}\begin{array}{rcl}#2\end{array}\end{equation}}
\newcommand{\pbar}{\bar p}
\newcommand{\xbar}{\bar x}
\newcommand{\xo}{x^{\scriptscriptstyle 0}}
\newcommand{\tbar}{\bar t}
\newcommand{\xbaro}{{\bar x}^{\scriptscriptstyle 0}}
\newcommand{\perturbj}{d_jp}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\vecM}{\mathbf{M}}
\newcommand{\vecY}{\mathbf{Y}}
\newcommand{\vecd}{\mathbf{d}}
\newcommand{\fractext}[2]{#1/#2}
\newcommand{\IE}{{\em i.e.}\xspace}
\newcommand{\tx}{^{\mathrm{th}}}
\newcommand{\Ave}[1]{{\mathbb E}[ #1]}
\newcommand{\BigAve}[1]{{\mathbb E} \big[ #1\big]}
\newcommand{\prob}[1]{\Pr\left[ #1\right]}
\newcommand{\refine}{ \prec_{\mathpzc{r}} }

\newtheorem{direction}{Direction}
\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
\newtheorem{observation}{Observation}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
%%\renewcommand{\qedsymbol}{{\Pisymbol{pzd}{113}}

%%\newenvironment{proof}{{\noindent\bf Proof.\ }}{\hfill{\Pisymbol{pzd}{113}}\vspace{0.1in}}
\newenvironment{proof-sketch}{{\noindent\bf Sketch of Proof.\ }}{\hfill{\Pisymbol{pzd}{113}}\vspace{0.1in}}

\newcommand{\angstroms}{\AA}
\newcommand{\sharpP}{\mbox{\#P}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\LP}{{\mathsf{LP}}}
\newcommand{\SDP}{{\mathsf{SDP}}}
\renewcommand{\deg}{\mathsf{deg}}
\newcommand{\Z}{\mbox{\bf Z}}
\newcommand{\buzz}[1]{\emph{#1}}
\newcommand{\pinput}[0]{{\bf Input:}}
\newcommand{\poutput}[0]{{\bf Output:}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\nbr}{\mathsf{Nbr}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\EA}{{\em et al.}\xspace}
\newcommand{\TB}{\vspace{-0.1ex}}\newcommand{\TiE}{\setlength{\itemsep}{-1ex}}
\newenvironment{TightItem}{\TB\TB\begin{itemize}\TiE}{\end{itemize}\TB}
\newenvironment{TightEnum}{\TB\TB\begin{enumerate}\TiE}{\end{enumerate}\TB}
\newenvironment{TightDesc}{\TB\TB\begin{description}\TiE}{\end{description}\TB}
\newcommand{\SB}{{\bf S}}
\newcommand{\BR}{{\bf R}}
\newcommand{\comment}[1]{}
\newtheorem{proposition}{Proposition}
\newtheorem{Def}{Definition}
\newcommand{\real}{\ensuremath{\mathcal{R}}}
\newcommand{\pint}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\partes}[1]{\ensuremath{\mathcal{P}(#1)}}
\newcommand{\norma}[1]{\ensuremath{\parallel \! \! #1 \! \! \parallel}}
\newcommand{\Norma}[1]{\ensuremath{\left\| #1 \right\|}}
\newcommand{\set}[2]{\ensuremath{ \{ #1|\:#2 \} }}
\newenvironment{epigrafe}
{\begin{list}{}{\setlength{\leftmargin}{0.4\textwidth}}\item \small }
{\end{list} \vspace{3ex} }
\newcommand{\derecha}[1]{\begin{flushright} \vspace{-2ex} #1 \end{flushright}}
\newcommand{\eX}[1]{{\bf E}[#1]}
\newcommand{\EG}{{\it e.g.}\xspace}
\newcommand{\FI}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\MiBTR}{{\sc Min-BTR}\xspace}
\newcommand{\MaBTR}{{\sc Max-BTR}\xspace}
\newcommand{\BTR}{{\sf BTR}\xspace}
\newcommand{\MED}{{\sc Med}\xspace}
\newcommand{\UVX}{{u\stackrel{x}{\Rightarrow} v}}
\newcommand{\VUX}{{v\stackrel{x}{\Rightarrow} u}}
\newcommand{\uvx}{{u\stackrel{x}{\to} v}}
\newcommand{\EC}{{\mathsf{E}_{\mathrm{fixed}}}}
\newcommand{\vpseudo}{{V_{\rm pseudo}}}
\newcommand{\GPVC}{{\sc Gpvc}\xspace}
\newcommand{\MiGPVC}{{\sc Min-GPVC}\xspace}
\newcommand{\MaGPVC}{{\sc Max-GPVC}\xspace}
\newcommand{\PVC}{{\sc Pvc}\xspace}
\newcommand{\ULP}{{\sc Ulp}\xspace}
\newcommand{\DLP}{{\sc Dlp}\xspace}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\h}{{\mathfrak{h}}}
\newcommand{\Gr}{{\mathfrak{G}}}
\newcommand{\Ed}{{\mathfrak{E}}}
\newcommand{\Ve}{{\mathfrak{V}}}
\newcommand{\MI}{\mbox{\sf MI}}
\newcommand{\APX}{\mathsf{APX}}
\newcommand{\SC}{{\sf SC}\xspace}
\newcommand{\PPI}{{\sc Ppi}\xspace}
\newcommand{\ODE}{{\sc Ode}}
\newcommand{\qip}{{\sc Qip}}
\newcommand{\SVD}{{\sc Svd}}
\newcommand{\PCA}{{\sc Pca}}
\newcommand{\CP}{{\sc Cp}}
\newcommand{\ALS}{{\sc Als}}
\newcommand{\Tucker}{{\sc Tucker}}
\newcommand{\promotes}{{\stackrel{0}{\to}}}
\newcommand{\pathpromotes}{{\stackrel{0}{\Rightarrow}}}
\newcommand{\inhibits}{{\stackrel{1}{\to}}}
\newcommand{\pathinhibits}{{\stackrel{1}{\Rightarrow}}}
\newcommand{\general}{{\stackrel{x}{\to}}}
\newcommand{\pathgeneral}{{\stackrel{x}{\Rightarrow}}}
\newcommand{\ttrue}{{\bf{true}}}
\newcommand{\ffalse}{{\bf{false}}}
\newcommand{\iif}{{\bf{if}}}
\newcommand{\tthen}{{\bf{then}}}
\newcommand{\eelse}{{\bf{else}}}
\newcommand{\ffor}{{\bf{for}}}
\newcommand{\wwhile}{{\bf{while}}}
\newcommand{\rreturn}{{\bf{return}}}
\newcommand{\rrepeat}{{\bf{repeat}}}
\newcommand{\ddo}{{\bf{do}}}
\newcommand{\xtc}{{\sc X3c}}
\newcommand{\bSC}{{\sc Sc}}
\newcommand{\sat}{{\sc Sat}}
\newcommand{\lgl}{{\sc Lgl}}

%%%%%%% new ones 
\newcommand{\gscaled}{\delta^{\mathrm{Y}}}
\newcommand{\Gscaled}{\Delta^{\mathrm{Y}}}
\newcommand{\gdiam}{\delta^{\mathrm{\cD}}}
\newcommand{\Gdiam}{\Delta^{\mathrm{\cD}}}
\newcommand{\diam}{\mathsf{diam}}
\newcommand{\gL}{\delta^{\mathrm{L}}}
\newcommand{\GL}{\Delta^{\mathrm{L}}}
\newcommand{\gLMS}{\delta^{\mathrm{L+M+S}}}
\newcommand{\GLMS}{\Delta^{\mathrm{L+M+S}}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\vol}{\mathsf{vol}}
\newcommand{\have}{\pmb{\overline{h}}}
\newcommand{\cut}{\mathrm{cut}}
\newcommand{\g}{\mathpzc{g}}
\newcommand{\wt}{\mathpzc{w}}
\newcommand{\muopt}{ \pmb{\mu_{\mathrm{opt}}} }
\newcommand{\opt}{ {\mathsf{OPT}} }
\newcommand{\nopt}{ {\mathsf{OPT}_{\#}} }
\newcommand{\lopt}{ \mathpzc{L}_{\mathrm{opt}} }
\newcommand{\loptgt}{ \mathpzc{L}_{\mathrm{opt}}^{\geq k} }
\newcommand{\lopteq}{ \mathpzc{L}_{\mathrm{opt}}^{=k} }
\newcommand{\lopteqone}{ \mathpzc{L}_{\mathrm{opt}}^{=1} }
\newcommand{\hatlopt}{ \widehat{ \mathpzc{L}_{\mathrm{opt}} } }
\newcommand{\hatlopteqone}{ \widehat{ \mathpzc{L}_{\mathrm{opt}}^{=1} } }
\newcommand{\hatloptgt}{ \widehat{ \mathpzc{L}_{\mathrm{opt}}^{\geq k} } }
\newcommand{\vopt}{ V_{\mathrm{opt}} }
\newcommand{\voptgt}{ V_{\mathrm{opt}}^{\geq k} }
\newcommand{\vopteq}{ V_{\mathrm{opt}}^{=k} }
\newcommand{\vopteqone}{ V_{\mathrm{opt}}^{=1} }
\newcommand{\vhat}{\widehat{V}}
\newcommand{\hatvopt}{ \widehat{ V_{\mathrm{opt}} } }
\newcommand{\hatvopteqone}{ \widehat{ V_{\mathrm{opt}}^{=1} } }
\newcommand{\hatvoptgt}{ \widehat{ V_{\mathrm{opt}}^{\geq k} } }
\newcommand{\hatkopt}{ \widehat{ k_{\mathrm{opt}} } }
\newcommand{\scopt}{ \mathsf{opt}_{\!\!\text{\footnotesize\sc Sc}\!\!}}
\newcommand{\xtcopt}{ \mathsf{opt}_{\!\!\!\text{\footnotesize\sc X3c}\!\!}}
\newcommand{\vspecial}{ v_{\mathrm{special} } }
\newcommand{\mds}{{\sc Mds}}
\newcommand{\mse}{{\sc Mse}}
\newcommand{\uumv}{{\sc Uumv}}
\newcommand{\hssc}{{\sc Hssc}}
\newcommand{\nokmad}{{\sc Adim}}
\newcommand{\mad}{{\sc Adim}$_{\geq k}$}
\newcommand{\eqmad}{{\sc Adim}$_{= k}$}
\newcommand{\eqmadone}{{\sc Adim}$_{= 1}$}
\newcommand{\eqonemad}{{\sc Adim}$_{=1}$}
\newcommand{\nhssc}{{\sc Nhssc}}
\newcommand{\mvap}{{\sc Mvap}}
\newcommand{\mvnp}{{\sc Mvnp}}
\newcommand{\ehslcp}{{\sc Ehslcp}}
\newcommand{\nhslcp}{{\sc Nhslcp}}
\newcommand{\minrep}{{\sc Minrep}}
\newcommand{\modclust}{{\sc Modclust}}
\newcommand{\sse}{{\sc Sse}}
\newcommand{\low}{\mathsf{low}}
\newcommand{\high}{\mathsf{high}}
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}
\newcommand{\sos}{{\sc Sos}}
\newcommand{\mwvp}{{\sc Min}-{\sc wvp}}
%%%%%%%%%%%%%%%
\definecolor{columbiablue}{rgb}{0.61, 0.87, 1.0}
\newcommand{\trueblue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\trueblack}[1]{{\textcolor{black}{#1}}}
\newcommand{\truegray}[1]{{\textcolor{gray}{#1}}}
\newcommand{\truegreen}[1]{{\textcolor{green}{#1}}}
\newcommand{\soln}{\mathsf{SOLUTION}}
\newcommand{\aalpha}{{\mathrm{PartyA}}}
\newcommand{\bbeta}{{\mathrm{PartyB}}}
\newcommand{\eeta}{{\mathrm{Pop}}}
%%\renewcommand{\k}{\mathscr{k}}
\newcommand{\fmc}{\textsc{Fmc}\xspace}
\newcommand{\nfmc}{\textsc{Node-fmc}\xspace}
\newcommand{\sfmc}{\textsc{Segr-fmc}\xspace}
\newcommand{\bfmc}{\ensuremath{\Delta}-\textsc{bal-fmc}\xspace}
\newcommand{\gfmc}{\textsc{Geom-fmc}\xspace}
%%\newcommand{\cpvc}{\textsc{Cpvc}\xspace}
\newcommand{\fmcg}[2]{\textsc{Fmc}(\ensuremath{#1, #2})}
\newcommand{\mindisc}{\textsc{Min-disc}\xspace}
%%%%%%%%%
%%%%%%%%%
\newcommand{\algmed}{\textsc{Alg}-\textsc{medium}-\textsc{opt}\ensuremath{_\#}\xspace}
\newcommand{\algsm}{\textsc{Alg}-\textsc{small}-\textsc{opt}\ensuremath{_\#}\xspace}
\newcommand{\algla}{\textsc{Alg}-\textsc{large}-\textsc{opt}\ensuremath{_\#}\xspace}
\newcommand{\algiter}{\textsc{Alg}-\textsc{iter}-\textsc{round}\xspace}
%%%%%%%%%
%%%%%%%%%
\newcommand{\optf}{\ensuremath{\opt_{\mathrm{frac}}}}
\newcommand{\optv}{\ensuremath{\opt_{\mathrm{SDP}}}}
\newcommand{\tf}{\ensuremath{t^{\mathrm{final}}}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\renewcommand{\b}{\mathbf{b}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\khat}{\ensuremath{\widehat{k}}}
\newcommand{\Ghat}{\ensuremath{\widehat{G}}}
\newcommand{\Vhat}{\ensuremath{\widehat{V}}}
\newcommand{\Ehat}{\ensuremath{\widehat{E}}}
\newcommand{\Xhat}{\ensuremath{\widehat{X}}}
\newcommand{\Yhat}{\ensuremath{\widehat{Y}}}
\newcommand{\phat}{\ensuremath{{\widehat{p}}}}
\newcommand{\qhat}{\ensuremath{{\widehat{q}}}}
\newcommand{\nhat}{\ensuremath{\widehat{n}}}
\newcommand{\mhat}{\ensuremath{\widehat{m}}}
\newcommand{\rhat}{\ensuremath{\widehat{r}}}
\newcommand{\Vsol}{\ensuremath{\Vhat_{\mathrm{sol}}}}
\newcommand{\Esol}{\ensuremath{\Ehat_{\mathrm{sol}}}}
\newcommand{\Xsol}{\ensuremath{\Xhat_{\mathrm{sol}}}}
\newcommand{\Ysol}{\ensuremath{\Yhat_{\mathrm{sol}}}}

\allowdisplaybreaks

\makeatletter
\def\namedlabel#1#2{\begingroup
    #2%
    \def\@currentlabel{#2}%
    \label{#1}\endgroup
}
\makeatother

%\usepackage[scr=bickham,scrscaled=1.05]{mathalfa}
\usepackage[scr=boondoxo]{mathalfa}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> exp.tex <==
% \begin{figure*}[!hb] 
%     \begin{minipage}[t]{0.49\linewidth}
%         	\centering
%         	\includegraphics[width=\textwidth]{plots/sampled_ranking/varying_size_prep_time.png} 
%         	\caption{Effect of varying dataset size on preprocessing time in the \ranker}
%          \label{fig:ranking_varying_size_prep_time}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.49\linewidth}
%         \centering
%         	\includegraphics[width =\textwidth]{plots/sampled_ranking/varying_size_unfairness.png} 
%         	\caption{Effect of varying dataset size on pairwise fairness before/after applying \ranker}\label{fig:ranking_varying_size_unfairness}
%     \end{minipage}
% \end{figure*}
\section{Experiments}
Besides theoretical analysis, We performed experiments under a variety of settings to confirm fairness and memory/time efficiency of our proposed algorithms. 
% To evaluate our algorithms for efficiency and effectiveness, We performed experiments under a variety of settings. 
The experiments were conducted on an Apple M2 processor with 16 GB of memory, running macOS. The algorithms were implemented in Python.
In our experiments, we used \textsc{Adult} dataset \cite{misc_adult_2}, a commonly used dataset in the fairness literature \cite{bellamy2018ai}, with column {\tt sex=\{male, female\}} as the sensitive attribute and {\tt fnlwgt} and {\tt education-num} columns with continuous real and discrete ordinal values for ordering the tuples. \textsc{Adult} dataset includes 15 census data related attributes with $\sim$49000 tuples describing people and is primarily used to predict whether an individual's income exceeds \$50K per year.
The default values are as following: bucket size=100, n=20000, and female-to-male ratio=0.25.

% \abol{what is the default number of buckets? }


\stitle{\ranker} We start our experiments by evaluating the \ranker algorithm.
Recall that this algorithm outputs an $(\optRank,1)$-hashmap and has a time complexity of $O(n^2\log n)$ in 2D.
% In our first experiment, instead of using the entire data set for identifying alternative rankings, we sampled subsets of the data set with various sizes. Still, we used the entire data set to measure the fairness of each ranking. 
In order to study the impact of $n$, in our first experiment, we vary the data set size by selecting different portions of the shuffled data set.
The results are provided in Figures~\ref{fig:ranking_varying_size_prep_time} and \ref{fig:ranking_varying_size_unfairness}.
First, in Figure~\ref{fig:ranking_varying_size_prep_time} one can confirm that, overall, the run-time increases as the size of the sample set increases. Still, the exact time depends on the number of rankings generated which depends on the value distributions on the selected samples.
Next, in Figure~\ref{fig:ranking_varying_size_unfairness} it is evident that, irrespective of the data set size, in all cases the output of \ranker had an unfairness (disparity) close to zero.


% \begin{wrapfigure}{r}{0.45\textwidth}
%     \centering
%     \vspace{-8mm}
%     \includegraphics[width =0.45\textwidth]{plots/sweep_n_cut/varying_ratio_space.png} 
%     \vspace{-10mm}
%         	\caption{Effect of varying the ratio of minority to majority on the number of cuts added by \pd}
%             \label{fig:sweep_varying_ratio_space}
%     \vspace{-13mm}
% \end{wrapfigure}

\stitle{\pd}
While \pd outputs a 0-unfair hashmap, its major draw back is memory since in worst-case it can create $O(n)$ cuts. Lemma~\ref{th:pd:mem:avg} provides an upper-bound on the expected number of cuts as a function of the minority ratio in the data set.
To evaluate how tight this upper-bound is in practice, in Figure~\ref{fig:sweep_varying_ratio_space}, we generate data set instances with various minority-to-majority ratios, and observe the actual number of cuts. At least in this experiment, the upper-bound was tight as it always less that 30\% larger than the actual number. The other observation is that \pd's memory requirement is indeed close to the worst case of $O(n)$ cuts.


% \begin{figure*}[h] 
%     \begin{minipage}[t]{0.49\linewidth}
%         \centering
%         	\includegraphics[width =\textwidth]{plots/necklace_splitting/varying_size_prep_time.png} 
%         	\caption{Effect of varying dataset size on preprocessing time in the \necklaceb}
%             \label{fig:necklace_varying_size_prep_time}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.49\linewidth}
%         	\centering
%         	\includegraphics[width =\textwidth]{plots/necklace_splitting/varying_size_space.png}
%         	\caption{Effect of varying dataset size on the number of cuts in the \necklaceb}
%             \label{fig:necklace_varying_size_space}
%     \end{minipage}
% \end{figure*}

\stitle{\necklaceb}
The number of cuts added by \necklaceb is independent of $n$ and is bounded by $2(m-1)$.
To experimentally verify these and observe the actual number of cuts added by the algorithm.
Figures~\ref{fig:necklace_varying_size_prep_time} and \ref{fig:necklace_varying_size_space}
show the run-time of \necklaceb and the number of cuts it introduced for each case over various data set sizes.
As expected, one can confirm the number of cuts is independent of $n$. Interestingly, the run-time of the algorithm also did not noticeably change as $n$ increased.

% \begin{figure*}[h] 
%     \begin{minipage}[t]{0.49\linewidth}
%         	\centering
%         	\includegraphics[width=\textwidth]{plots/necklace_splitting/varying_num_of_buckets_prep_time.png} 
%         	\caption{Effect of varying the number of buckets on the preprocessing time in the \necklaceb}
%             \label{fig:necklace_varying_num_of_buckets_prep_time}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.49\linewidth}
%         \centering
%         	\includegraphics[width =\textwidth]{plots/necklace_splitting/varying_num_of_buckets_space.png} 
%         	\caption{Effect of varying the number of buckets on the number of cuts in the \necklaceb}
%             \label{fig:necklace_varying_num_of_buckets_space}
%     \end{minipage}
% \end{figure*}

Next, in Figures~\ref{fig:necklace_varying_num_of_buckets_prep_time} and Figure~\ref{fig:necklace_varying_num_of_buckets_space}, we vary the number of buckets from 100 to 1000.
The time complexity of \necklaceb is $O(n\log n)$. As a result, varying $m$ should not impact its run-time, which is consistent with our experiment results in Figure~\ref{fig:necklace_varying_num_of_buckets_prep_time}.
The number of cuts, however, are guaranteed to be at most $2(m-1)$. Interestingly, in almost all settings in Figure~\ref{fig:necklace_varying_num_of_buckets_space}, the actual number of cuts was close to the upper-bound.


\begin{comment}
% \input{plots}
\subsection{Efficiency}
\paragraph{Time}
We begin our evaluation by studying the impact of input size on the preprocessing time in \ranker algorithm. As demonstrated in Figure \ref{fig:ranking_varying_size_prep_time}, as the input size grows, the number of rankings and eventually the preprocessing time increase.
Furthermore, as shown in Figure \ref{fig:ranking_varying_num_of_buckets_prep_time}, as the number of buckets increases, the number of boundaries and hence the number of rankings to be reevaluated also grow which results in an increased preprocessing time. Next, by looking at Figure \ref{fig:necklace_varying_size_prep_time} and comparing the results with the \ranker algorithm, we observe the superiority of \necklaceb in terms of significantly lower preprocessing time. Moreover, despite the \ranker, as shown in Figure \ref{fig:necklace_varying_num_of_buckets_prep_time}, increasing the number of buckets does not affect the preprocessing time in \necklaceb algorithm.
\paragraph{Space}
We start by evaluating the impact of varying dataset size on the space in \necklaceb algorithm. Figure \ref{fig:necklace_varying_size_space} indicates the independence of number of cuts from the input size in \necklaceb algorithm. Next, we vary the number of buckets and as demonstrated in Figure \ref{fig:necklace_varying_num_of_buckets_space} observe the linear correlation with the number of cuts with the values being closer to the upper-bound in all cases. Finally as presented in Figure \ref{fig:sweep_varying_ratio_space} and Lemma \ref{th:pd:mem:avg} , \pd shows a linear increase in the number of cuts as the ratio of of the majority to minority groups gets closer to 1.  
\subsection{Effectiveness}
Although \ranker-based algorithms do not provide guarantees on the zero unfairness, as illustrated in Figures \ref{fig:ranking_varying_size_unfairness} and \ref{fig:ranking_varying_ratio_unfairness}, they achieve insignificant disparity values between the majority and minority groups from a pairwise fairness perspective compared to the fairness-agnostic hashmap.
\end{comment}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> plots.tex <==
\begin{figure*}[!ht] 
    \begin{minipage}[t]{0.32\linewidth}
        	\centering
        	\includegraphics[width=\textwidth]{plots/sampled_ranking/varying_size_prep_time.png} 
        	\caption{Effect of varying dataset size on preprocessing time in the \ranker}
            \label{fig:ranking_varying_size_prep_time}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        	\includegraphics[width =\textwidth]{plots/sampled_ranking/varying_size_unfairness.png} 
        	\caption{Effect of varying dataset size on pairwise fairness before/after applying \ranker}
            \label{fig:ranking_varying_size_unfairness}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        	\centering
        	\includegraphics[width =\textwidth]{plots/sampled_ranking/varying_ratio_unfairness.png}
        	\caption{Effect of varying the ratio of majority to minority on pairwise fairness before/after applying \ranker}
            \label{fig:ranking_varying_ratio_unfairness}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        	\centering
        	\includegraphics[width=\textwidth]{plots/sampled_ranking/varying_num_of_buckets_prep_time.png} 
        	\caption{Effect of varying number of buckets on preprocessing time in the \ranker}
            \label{fig:ranking_varying_num_of_buckets_prep_time}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        	\includegraphics[width =\textwidth]{plots/necklace_splitting/varying_size_prep_time.png} 
        	\caption{Effect of varying dataset size on preprocessing time in the \necklaceb}
            \label{fig:necklace_varying_size_prep_time}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        	\centering
        	\includegraphics[width =\textwidth]{plots/necklace_splitting/varying_size_space.png}
        	\caption{Effect of varying dataset size on the number of bins in the \necklaceb}
            \label{fig:necklace_varying_size_space}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        	\centering
        	\includegraphics[width=\textwidth]{plots/necklace_splitting/varying_num_of_buckets_prep_time.png} 
        	\caption{Effect of varying the number of buckets on the preprocessing time in the \necklaceb}
            \label{fig:necklace_varying_num_of_buckets_prep_time}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        	\includegraphics[width =\textwidth]{plots/necklace_splitting/varying_num_of_buckets_space.png} 
        	\caption{Effect of varying the number of buckets on the number of bins in the \necklaceb}
            \label{fig:necklace_varying_num_of_buckets_space}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        	\includegraphics[width =\textwidth]{plots/sweep_n_cut/varying_ratio_space.png} 
        	\caption{Effect of varying the ratio of majority to minority on preprocessing time in \pd}
            \label{fig:sweep_varying_ratio_space}
    \end{minipage}
\end{figure*}   

==> prelimAppndx.tex <==
\section{Additional Preliminaries}
\label{appndx:prelim}

\stitle{Ensuring Pareto-optimality}
A major challenge when formulating fair algorithms is that those may generate Pareto-dominated solutions~\cite{nilforoshan2022causal}. 
That is, those may produce a fair solution that are worse for all groups, including minorities, compared to the unfair ones.
In particular, in a utility assignment setting, let the utility assigned to each group $\gee_i$ by the fair algorithm be $u_i$. There may exist another (unfair) assignment that assigns $u'_i>u_i$, $\forall \gee_i\in \Gee$.
This usually can happen when fairness is defined as the parity between different groups, without further specifications.

In this paper, the requirements 2 and 3 (single and pairwise fairness) have been specifically defined in a way to prevent generating Pareto-dominated fair solutions.
To better explain the rational behind our definitions, let us consider pairwise fairness (the third requirement). Only requiring equal collision probability between various groups, the fairness constraint would translate to $Pr[\hashfunction(p_i)=\hashfunction(q_i)]= Pr[\hashfunction(p_k)=\hashfunction(q_k)]$, where $p_i$ and $q_i$ belong to group $\gee_i$.
Now let us consider a toy example with two groups $\{\gee_1,\gee_2\}$,  two buckets $\{b_1,b_2\}$, and $n$ points where half belong to $\gee_1$. Let the hashmap $\hashmap$ map each point $p\in \gee_1$ to $b_1$ and each point $q\in\gee_2$ to $b_2$.
%, as illustrated in the following.
%
%\begin{center}
%\begin{tabular}{c|c|c|c}
    % {\tt \small bucket}& $\gee_1$&$\gee_2$&$|b_i|$  \\ \hline
     %$b_1$&$\frac{n}{2}$&0& %$\frac{n}{2}$ \\ \hline
     %$b_2$&0&$\frac{n}{2}$& %$\frac{n}{2}$ \\
%\end{tabular}
%\end{center}
%
In this example, the collision probability between a random pair of points is 0.5, simply because each bucket contains half of the points.
It also satisfies the collision probability equality between pairs of points from the same groups:
$Pr[\hashfunction(p_i)=\hashfunction(q_i)]= Pr[\hashfunction(p_k)=\hashfunction(q_k)] = 1$.

This, however, is the worst assignment for both groups as their pairs {\em always collide}. In other words, it is fair, in a sense that it is equally bad for both groups. Any other hashmap would have a smaller collision probability for both groups and, even if not fair, would be more beneficial for both groups.
In other words, this is a fair but Pareto-dominated solution.

In order to ensure Pareto-optimality while developing fair hashmaps, in requirements 2 and 3 (single and pairwise fairness), not only we require the probabilities to be equal, but also we require them to be equal to the {\em best case}, where the collision probability is $\frac{1}{m}$. As a result, we guarantee that (1) our hashmap is fair and (2) no other hashmap can do better for any of the groups.

\begin{comment}
\stitle{Calculation of probabilities}
Given a hashmap, we give the exact close forms for computing the collision probability, the single fairness, and the pairwise fairness.
Let $\alpha_{i,j}$ be the number of items from group $i$ at bucket $j$ and let $n_j=\sum_{i=1}^k\alpha_{i,j}$.
The probabilities are calculated as following,
collision probability: $\sum_{j=1}^m\left(\frac{n_j}{n}\right)^2$, single fairness: $\sum_{j=1}^m\frac{\alpha_{i,j}}{|\gee_i|}\cdot \frac{n_j}{n}$, pairwise fairness: $\sum_{j=1}^m\left(\frac{\alpha_{i,j}}{|\gee_i|}\right)^2$.
\end{comment}

==> rishi-header.tex <==
%% Compatibility, layout, and typography %%
\usepackage{lmodern}  % improves display of text
\usepackage[T1]{fontenc}  % allows LaTeX to output non-ASCII characters better; load after fonts if possible
\usepackage[english]{babel}  % sets language to American English
%\usepackage{csquotes}  % for formal quotations
\usepackage{fullpage}  % 1-inch margins all around
\usepackage{titling}  % can be used to create a title page
\usepackage{caption}  % fixes table--caption spacing in article class
\frenchspacing
\usepackage{microtype}  % improves typographic details (e.g., kerning)
\usepackage{fnpct}  % adjusts kerning of footnote marks (superscripts) before commas or periods


%% Bibliography %%
\usepackage[numbers, sort&compress]{natbib}
\bibliographystyle{plainnat}


%% Images %%
\usepackage{graphicx}  % allows inclusion of images in document
\graphicspath{{./images/}}  % location of images in file system

% Example:
%\begin{figure}[bhpt]
%\centering
%\includegraphics[width=0.8\linewidth]{p1_1}
%\caption{[insert caption]}
%\label{p1_relevantname}
%\end{figure}


%% Tables %%
\usepackage{booktabs}
%\usepackage{tabularx}


%% Math %%
\usepackage{mathtools, amssymb, amsthm}  % mathtools loads amsmath

\allowdisplaybreaks[1]  % allows page breaks within amsmath environments; optional value from 1-4 sets permissibility (4 being the highest)

% \mathchardef\mhyphen="2D  % hyphen for math mode (credit to Gernot Salzer)
\renewcommand*{\emptyset}{\varnothing}  % prettier empty set symbol
\usepackage{bm}  % use \bm for bold math symbols

% Use \phanrel to insert an invisible relation operator to align an equation split across two lines.
\newcommand*{\phanrel}{\mathrel{\phantom{=}}}
% Example:
% \begin{align*}
%     &\phanrel \text{a very long expression} \\
%     &= \text{another long expression}
% \end{align*}

\newcommand*{\Complex}{\mathbb{C}}
\newcommand*{\Reals}{\mathbb{R}}
\newcommand*{\Rationals}{\mathbb{Q}}
\newcommand*{\Integers}{\mathbb{Z}}
\newcommand*{\Naturals}{\mathbb{N}}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% Use \set for set notation. Starred version \set* automatically resizes with contents.
\DeclarePairedDelimiterX\set[1]\lbrace\rbrace{\,\def\suchthat{\;\delimsize|\;}#1\,}
% Example:
% $\set{x \suchthat x > 0}$

\newcommand*{\greedy}[1]{{\small $\textsc{Greedy}_{#1}$}}


%% Graphs %%
\usepackage{tikz}
\usetikzlibrary{babel, positioning}


%% Algorithms %%
% \usepackage{algorithm}  % needed to float algorithms
% \usepackage{algpseudocode}  % loads algorithmicx package as well; use option ``noend'' to supress block ending lines
% \newcommand*{\algorithmautorefname}{Algorithm}  % for hyperref's autoref macro

% Use \LongState to replace \State when the contents of the line overflow. This preserves the indentation level of the first line.
% \newcommand*{\LongState}[2]{\State\parbox[t]{\dimexpr\linewidth-\dimexpr\algorithmicindent*#1}{#2\strut}}  % inspired by a macro designed by TeX.SX user Werner
% Example:
% \LongState{2}{very long line that needs to be indented 2 levels}


% Use \isitdefined to check if a command is defined.
\newcommand*{\isitdefined}[1]{\%\% command `#1' does \ifcsname#1\endcsname\else NOT \fi exist \%\%}
% Example:
% \isitdefined{potato}


%% Load last %%
\usepackage[colorlinks, allcolors=blue]{hyperref}  % enable hyperlinks; load before `ellipsis`
\hypersetup{
    pdfinfo={
        Title={Online Maximum Independent Set of Hyperrectangles},
        Author={Anonymous author(s)},  % TODO update for arXiv submission
        Keywords={maximum independent set; hyperrectangle; geometric intersection graph; online algorithm; competitive ratio; adversary model}
    }
}
\usepackage{ellipsis}  % adjusts spacing of ellipses before punctuation
